Adaptive shape optimization with NURBS designs and PHT-splines for solution approximation in time-harmonic acoustics

Geometry Independent Field approximaTion (GIFT) was proposed as a generalization of Isogeometric analysis (IGA), where different types of splines are used for the parameterization of the computational domain and approximation of the unknown solution. GIFT with Non-Uniform Rational B-Splines (NUBRS) for the geometry and PHT-splines for the solution approximation were successfully applied to problems of time-harmonic acoustics, where it was shown that in some cases, adaptive PHT-spline mesh yields highly accurate solutions at lower computational cost than methods with uniform refinement. Therefore, it is of interest to investigate performance of GIFT for shape optimization problems, where NURBS are used to model the boundary with their control points being the design variables and PHT-splines are used to approximate the solution adaptively to the boundary changes during the optimization process. In this work we demonstrate the application of GIFT for 2D acoustic shape optimization problems and, using three benchmark examples, we show that the method yields accurate solutions with significant computational savings in terms of the number of degrees of freedom and computational time.

==> Sections/Methods/BEM.tex <==
Nowadays, the boundary element method (BEM) is a well-established numerical method, used in many areas of engineering and mathematical physics (see e.g. \cite{BEM_review} for a detailed review) with several open-access libraries and software available for general analysis and research purposes (e.g. \cite{BEM_web}). First works on BEM date back to 1960s, for example, in \cite{Jones_BEM} a 2D integral equation of potential theory was solved by discretizing the boundary and the solution with linear and constant elements respectively. In the following years, applications of BEM were extended to such areas as linear elasticity \cite{Rizzo_elasticity_BEM}, acoustics \cite{BEM_acoustics_early}, electromagnetics and many others, \cite{Paris_BEM_book}. A comprehensive overview of the heritage and history of BEM can be found in \cite{heritage_BEM}.    

The boundary element method is one of the family of methods based on the integral representation of solutions of boundary value problem (\ref{eq:1}) - (\ref{eq:4}). First, it requires the fundamental solution $G(x, x_0)$ of the governing (Helmholtz) equation, i.e. its solution for $f = \delta(x-x_0)$. Next, if the solution is represented as a combination of integrals with $G(x, x_0)$ and $\dfrac{\partial G(x, x_0)}{\partial n}$ (the so-called single and double layer potentials), then it satisfies the Helmholtz equation everywhere in the domain and the boundary condition is formulated as a boundary integral equation (BIE) for unknown $u$ or $\dfrac{\partial u}{\partial n}$ on the boundary, \cite{Kress_book}, \cite{KRESS1991229}. 

Boundary element method (BEM) is the method of discretizating the boundary integral equations, either in the context of collocation or variational (Galerkin) method, \cite{acoustic_bem_book}. Conventional BEM employs Lagrange polynomials as shape functions, \cite{Brebbia_BEM_book}. More recent versions employ splines, such as NURBS, \cite{SIMPSON2014265}.

In comparison with domain type methods like FEM, BEM presents a number of advantages:

1. The dimensionality of the problem is reduced by one. It means that only discretization of the boundary is required. It significantly reduces the computational effort for large domains. 

2. In exterior domains, asymptotic behaviour of solutions at infinity (known as Sommerfeld radiation condition in acoustics) is automatically satisfied due to the properties of $G(x, x_0)$ and $\dfrac{\partial G(x, x_0)}{\partial n}$ in the integral representation. It allows to avoid domain truncation error, discussed in Chapter \ref{trunc-domain-chapter}.

3. Due to the integral representation of solutions, the method is highly accurate in handling domains with sharp corners and other singularities. For example, it is widely applied in computational fracture mechanics to model cracks, \cite{Peng201755}. The coincident crack faces are modelled in the framework of the so-called dual BEM, which consists in prescribing BIEs of two different types, singular and hypersingular, on different crack faces \cite{Portela1992TheDB}. In the context of acoustics, similar approach is used to deal with coincident boundaries, e.g. in \cite{SHAABAN2022108410} it is used to model thin inner walls of a muffler, as well as overcome the spurious eigenfrequency problem, which appear in the exterior problems. The latter is known as Burton-Miller equation \cite{Burton-Miller-BEM}. 

However, BEM presents a few major drawbacks: 

1. First drawback is associated with the lack of fundamental solutions for some complex applications, such as non-homogeneous, non-linear and coupled problems. Application of BEM in some cases is still possible but requires complicated and problem dependent modifications \cite{KATSIKADELIS1999365}.   

2. If the problem has a domain source, the boundary integral equation contains a domain term and therefore loses its boundary-only nature and requires treatment of domain integrals. Some remedies include decomposition of the domain source into simpler terms, which can be integrated directly, \cite{YU2021113197}.  

3. The system matrices in BEM are dense and non-symmetric, hence, the computational complexity of the method with respect to the number of DOFs is said to be $O(N^2)$. Therefore, the use of BEM for large-scale problem is limited by the storage requirements and solution time of linear algebra solvers for full systems. The most popular approach to accelerate the matrix assembly and inversion in BEM is the so-called fast-multipole method (FMM), first proposed in \cite{gr86}. The main idea of FMM-BEM consists in introducing the multipole and local expansions of the fundamental solutions which enable computing integrals on clusters of far-field elements instead of on each element individually. The approach has been successfully employed in acoustic BEM, e.g. in \cite{Chen-FMM-BEM}.

3. The necessity to integrate singular integrals that appear in BEM kernels is also regarded as a challenge. However, some very efficient methods, such as regularization of BIEs \cite{Tanaka_regularization} and singularity subtraction techniques \cite{Guiggiani_SST}, have been proposed and are widely used for BIE with various orders of singularity. 

==> Sections/Methods/Domain-trunc-error.tex <==
When an exterior boundary value problem is solved by a domain-type method, the computational domain needs to be truncated by an artificial boundary (typically a circle in 2D and a sphere in 3D, with radius $R$). On the truncation boundary, the so-called Absorbing Boundary Condition (ABC) is prescribed. The ABC represents an assymptotic expansion of the Sommerfield radiation condition and hence introduces an additional error into the solution. This error is referred as a domain truncation error. Domain truncation error depends on the size of the domain, i.e. radius $R$, and decreases as $R$ grows. However, increasing $R$ leads to increasing the number of DOFs and the size of the system, and as a consequence, increasing the computational cost.

Another possibility to reduce the domain truncation error is to increase the order of the ABC. In this work, we use ABCs of the BGT type, originally introduced in \cite{Bayliss1980} and \cite{BGT_main}. Various approach to derive the ABCs are compared in \cite{ZARMI2013387}. The ABCs are written as 
\begin{equation}
\mathcal{B}^{(m)}u = 0, \label{BGTn}
\end{equation}
where $\mathcal{B}^{(m)}$ is the differential operator of order $m$, given in the polar coordinates by
\begin{equation}
    \mathcal{B}^{(m)}(\cdot) = \prod\limits_{j = 1}^m \left\{\dfrac{\partial (\cdot)}{\partial r} + \left(\dfrac{2 j -\frac{3}{2}}{r} - i k\right) (\cdot)\right\} \text{   in 2D}\label{B_n_2D}
\end{equation}
and 
\begin{equation}
    \mathcal{B}^{(m)}(\cdot) = \prod\limits_{j = 1}^m \left\{\dfrac{\partial (\cdot)}{\partial r} + \left(\dfrac{2 j -1}{r} - i k\right) (\cdot)\right\} \text{   in 3D} \label{B_n_3D}
\end{equation}

As can be seen from eq. (\ref{B_n_2D}) and (\ref{B_n_3D}), the ABCs contain derivatives of order $m$ and hence require higher order shape functions to accurately approximate them. This is regarded as a bottleneck of the traditional linear FEM, but can be achieved in the framework of IGA and GIFT with splines of sufficiently high order and continuity. 

Another family of ABCs are the so-called farfield expansion (FFE) absorbing boundary conditions (known as Karp’s Double and Single Farfield Expansions in 2D and Wilcox’s Farfield Expansionsin 3D. These ABCs are discussed in detail in \cite{VILLAMIZAR2017331} and implemented in the framework of IGAFEM in \cite{KHAJAH2019477}, in the framework of p-FEM in \cite{dsouza:hal-02540572} and in the framework of IGA-C in \cite{Atr-IGA-C}. The main idea of the FFE ABC is to decompose the asymptotic form of the solution at infinity in a series with known behavior in radial direction and unknown circumferential terms (in polar coordinates). As for any series, its accuracy increases as the number of terms is increased. Hence, a family of new unknown boundary functions is introduced, which needs to be discretized in addition to the solution inside the domain. This introduces additional DOFs, and as a consequence, leads to larger system and higher computational costs.  

Therefore, the goal of numerical analysis in an exterior domain is to have domain truncation error smaller than the discretization error, and also to achieve this for a reasonably small $R$. This is done by an appropriate choice of $R$, the order of the ABC and the mesh size, as demonstrated in the numerical studies in Chapter \ref{Num-Res}.  



==> Sections/Methods/IGA_lit_review.tex <==
The Finite Element Method (FEM) \cite{zienkiewicz1977finite} is the most popular and commonly employed method for numerical simulations in engineering applications. The full workflow in FEM is that first, designers produce a Computer-Aided Design (CAD) model of the object/structure that wants to be studied and then, engineers performs the analysis by the FEM. In a typical engineering scenario, the design is encapsulated in a CAD data-file, and the FEM analysis is performed over a discretization of that aforementioned CAD data, which is known as the mesh. In some instances, the mesh generation can be done automatically, but in most circumstances, it can be done at best semi-automatically, requiring several iterations in the mesh generation process. There are still situations in major industries where drawings are made of CAD designs, and meshes are built from them. It is estimated that about 80\% of overall analysis time is devoted to mesh generation in the automotive, aerospace, and shipbuilding industries \cite{hughes2005isogeometric}.

Hughes et al. \cite{hughes2005isogeometric} proposed back in 2005 the Isogeometric Analysis (IGA). This methods aims to merge both the design and analysis process by employing the same basis functions that are employed in the CAD design, usually given by NURBS curves, as the basis functions to solve the boundary value problem. 

Over ten years of development has made IGA one of the most active research topics in both Computational Mechanics and Computer-Aided geometry design \cite{structural_shape_opt_review}. Advantages such as the exact representation of the geometry, higher continuity of the basis functions, natural operations for the degree elevation and knot insertion, among others, makes IGA superior to the conventional FEM.

Related to the wave equation, different works \cite{COOX2016441,WU201563,khajah2019b} have shown the superiority of IGA over others approach, especially when it comes to reducing the pollution error. The pollution error  \cite{babuska1997pollution,IHLENBURG19959, babushka_II} is a well-known phenomenon that affects the quality of the numerical solution when the size of the elements is not small enough to compensate the high frequency of the wave. IGA based method to solve the wave equation has proved to perform better compared to its FEM counterpart, but still, the pollution error is present in them.
Furthermore, plane-wave enriched IGA have shown even better results in terms of error versus degrees of freedom \cite{DINACHANDRA2018380,DIWAN2019701}.

One of the main drawbacks of IGA is that NURBS basis functions lacks a local refinement algorithm, which makes them  computationally highly expensive in applications that demands a non-uniform refinement of the geometry, such as problems with complex geometries or singularities. Different alternatives to NURBS, such as T-splines \cite{sederberg2003t,sederberg2004t}, PHT-Splines \cite{deng2006dimensions, deng2008polynomial}, and RPHT-splines \cite{wang2011adaptive} among others, allow adaptive refinement, and have been successfully applied within the IGA framework \cite{isogeometricTsplines1,isogeometricTsplines0,isogeometricTsplines2,ghorashi2015t,wang2011adaptive, nguyen2011isogeometric, nguyen2014adaptive,nguyen2011rotation,nguyen2017extended}. 

Atroshchenko et al. \cite{atroshchenko2018weakening} proposed GIFT as a numerical method that aims to decouple the field space from the geometry space. The field-geometry decoupling is achieved by using a more suitable basis function for the field space while keeping the exact representation of the geometry by NURBS. This method aims to employ the best basis function according to any particular characteristic of the problem (such as complex geometries or numerical singularities in the solution). The method has been successfully applied in problems of Linear elasticity \cite{atroshchenko2018weakening}, acoustics \cite{videla2019h}, fracture mechanics of Kirchhoff-Love plates \cite{videlaapplication}, vibration of Reissner-Mindlin plates \cite{yu2018adaptive}.  

Videla et al. \cite{videla2019h} showed the advantages of pairing PHT-splines with NURBS by GIFT in the context of time-harmonic problems. In particular, problems with local gradients given by geometrical irregularities can take advantage of the adaptive refinement given by PHT-splines, and achieve optimal convergence rates in the error norm, while keeping a course geometry and therefore saving computational resources.

==> Sections/Methods/NURBS.tex <==
Non-Uniform Rational B-splines (NURBS) are one of the most popular geometrical representations employed on the CAD/CAM industry. Introduced by Verspirlle in his doctoral dissertation \cite{versprille1975computer} back in 1975, NURBS quickly started being adopted by various companies and has consolidated as an industry standard when it comes to computer modelling. Further details on NURBS can be found on Piegl's survey \cite{nurbs_survey_piegl_1991} and subsequent book on NURBS \cite{nurbs_survey_piegl_1991}, whereas an introduction with a historical perspective can be found on \cite{rogers2001introduction}. 

IGA book \cite{hughes2005isogeometric}

Let $\Xi= \left \{ \xi_{0},...,\xi_{n+p+1} \right \} $ be a non-decreasing sequence of real numbers, i.e., $\xi_{i}<\xi_{i+1}$ with the sub-index $i=0,...,n+p+1$. The $\xi_{i}$ are called knots and $\Xi$ is called the knot vector, $n$ is the number of basis functions which comprise the NURBS and $p$ is the polynomial order of the NURBS. If knots are equally-spaced in the parametric space, they are said to be \textit{uniform}. If they are unequally spaced, then they are \textit{non-uniform}.

A $p$-th degree NURBS curve is defined by:

\begin{equation}
    C(\xi)=\sum_{i=1}^{n}R_{i,p}(\xi)\mathbf{P_{i}}
\label{NURBS curve}
\end{equation}

\noindent where ${\mathbf{P_{i}}}$ are the control points of the curve and $R_{i,p}$ are the Rational basis functions, defined by:

\begin{equation}
    R_{i,p}(\xi)=\frac{N_{i,p}(\xi)w_{i}}{\sum_{j=0}^{n}N_{j,p}(\xi)w_{\hat{j}}}
\end{equation}

\noindent where $w_{i}$  are the weights associated to each $ R_{i,p}(\xi)$ and $N_{i,p}(\xi)$ are the $p$-th degree B-Spline basis functions, which are defined in a recursive way:

\begin{equation*}
    N_{i,0}(\xi)=\left\{\begin{matrix}1 & \text{ if $\xi_{i}<\xi<\xi_{i+1}$}
\\ 
0 & \text{ otherwise}
\end{matrix}\right.
\end{equation*}
\begin{equation}
    N_{i,p}(\xi)=\frac{\xi-\xi_{i}}{\xi_{i+1}-\xi_{i}}N_{i,p-1}(\xi)+\frac{\xi_{i+p+1}-\xi}{\xi_{i+p+1}-\xi_{i+1}}N_{i+1,p-1}(\xi)
\end{equation}

 Figure \ref{fig:nurbs curve} shows an example of a 2D cubic NURBS curve with their control points. This curve is created with the following knot vector: $\Xi=\left \{ 0,0,0,0,0.4,0.5,0.6,1,1,1,1\right \}$. The control points are given on Table \ref{NURBS_curve_control_points_ex}, and the respective basis functions are shown on Figure \ref{fig:nurbs basis example}
 
 \begin{table}[ht!]
 \centering
\begin{tabular}{ccc}
\hline
\multicolumn{3}{l}{Control Points $P_i$} \\ \hline
$x$       & $y$       & $w$              \\ \hline
-4      & -4      & 1              \\
-4      & 0       & $\sqrt{2}/2$      \\
0       & 0       & 1              \\
0       & 4       & $\sqrt{2}/2$      \\
4       & 4       & 1              \\
4       & 0       & 1              \\
2       & -4      & 1             
\end{tabular}
\caption{NURBS curve: Control points and their respective weights}
\label{NURBS_curve_control_points_ex}
\end{table}

\begin{figure}[ht!]
\centering        
\includegraphics[width=0.5\textwidth]{Sections/Methods/images/nurbs_curve_example.eps}
\caption{NURBS curve in 2D: curve (blue line) and control points (red dots)}
%Source: \cite{hughes2005isogeometric}.
\label{fig:nurbs curve}
\end{figure}

\begin{figure}[ht!]
\centering        
\includegraphics[scale=0.8]{Sections/Methods/images/nurbs_basis_functions_curve.eps}
\caption{NURBS basis functions of Figure \ref{fig:nurbs curve}}
\label{fig:nurbs basis example}
\end{figure}

Analogously, a NURBS surface of $p$-th degree in the $\xi$ direction and $q$-th degree in the $\eta$ direction is defined by:

\begin{equation}
\mathbf{S}(\xi,\eta)=\sum_{i=1}^{n}\sum_{j=1}^{m}R_{i,j}^{p,q}(\xi,\eta)\mathbf{P_{ij}}
\end{equation}

\noindent where $\mathbf{P_{ij}}$ is a set of $n\times m$ bidirectional control net and $R_{i,j}^{p,q}$ is defined by:
\begin{equation}
R_{i,j}^{p,q}(\xi,\eta)=\frac{N_{i,p}(\xi)M_{j,q}(\eta)w_{i,j}}{\sum_{\hat{i}}^{n}\sum_{\hat{j}}^{m}N_{\hat{i},p}(\xi)M_{\hat{j},q}w_{\hat{i},\hat{j}}}
\label{eq: nurbs surface}
\end{equation}

\noindent where $N_{\hat{i},p}(\xi)$ and $M_{\hat{j},q}(\eta)$ are B-splines functions defined on knots sets  $\Xi_{1}$ and $\Xi_{2}$, respectively.

Figure \ref{fig:nurbs surface example} shows an example of a 2D linear-quadratic NURBS surface. The polynomial order and knot vectors are given on Table \ref{NURBS_surface_knot_table}, while the control points are shown on Table \ref{NURBS_surface_control_points_ex}. Figure \ref{basis_functions} shows the basis functions expanded over the aforementioned surface. 


\begin{figure}[ht!]
\centering        
\includegraphics[width=0.75\textwidth]{Sections/Methods/images/nurbs_surface_example.png}
\caption{NURBS surface in 2D: curve (blue line) and control points (red dots)}
\label{fig:nurbs surface example}
\end{figure}

\begin{table}[ht!]
\centering
\begin{tabular}{lll}
\hline
Direction           & Order & Knot Vector \\ \hline
$\xi$  & $p=1$   &  $\Xi=\left \{ 0,0,1,1\right \}$.           \\
$\eta$ & $q=2$   & $\Xi=\left \{ 0,0,0,1,1,1\right \}$           
\end{tabular}
\caption{NURBS surface: Polynomial orders and knot vectors for the surface shown in Figure \ref{fig:nurbs surface example}}
\label{NURBS_surface_knot_table}
\end{table}


\begin{table}[ht!]
\centering
\begin{tabular}{ccc}
\hline
\multicolumn{3}{l}{Control Points $P_{ij}$} \\ \hline
$x$          & $y$         & $w$         \\ \hline
1          & 0         & 1         \\
$\sqrt{2}/2$  & $\sqrt{2}/2$ & $\sqrt{2}/2$ \\
0          & 1         & 1         \\
2          & 0         & 1         \\
$\sqrt{2}$    & $\sqrt{2}$   & $\sqrt{2}/2$ \\
0          & 2         & 1        
\end{tabular}
\caption{NURBS surface: Control points and their respective weights for the surface shown in Figure \ref{fig:nurbs surface example}}
\label{NURBS_surface_control_points_ex}
\end{table}


\begin{figure}[ht!]
    \centering

    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Sections/Methods/images/nurbs_surface_basis_1.eps}
        \caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Sections/Methods/images/nurbs_surface_basis_2.eps}
        \caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Sections/Methods/images/nurbs_surface_basis_3.eps}
        \caption{}
    \end{subfigure}
    ~
  \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Sections/Methods/images/nurbs_surface_basis_4.eps}
        \caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Sections/Methods/images/nurbs_surface_basis_5.eps}
        \caption{}
    \end{subfigure}
    ~ 
    \begin{subfigure}[b]{0.45\textwidth}
        \includegraphics[width=\textwidth]{Sections/Methods/images/nurbs_surface_basis_6.eps} 
        \caption{}
    \end{subfigure}
    \caption{NURBS basis functions of the surface on Figure \ref{NURBS_surface_control_points_ex}. Each basis functions is plotted over the geometrical space}
\label{basis_functions}
\end{figure}

\clearpage

The B-spline basis functions have the following properties:

\begin{itemize}
    \item Linear independence. 
    \item Partition of unity.
    \item Compact support for each $N_{i,p}$in the interval $[ u_{i},u_{i+p+1}]$.
    \item Non-negative basis functions.
\end{itemize}


Since NURBS are transformations of the B-spline basis functions they inherit their main properties and obtain more. Some of them include:

\begin{itemize}
     \item Partition of unity.
     \item Continuity and support of B-spline.
     \item Affine transformations in a physical space are achieved by applying them to the control points. This means NURBS have the property of affine covariance.
     \item If the weights of all control points are equal, NURBS become B-splines.
\end{itemize}


==> Sections/Methods/PHT.tex <==
Polynomial Splines over hierarchical T-meshes (PHT-Splines) where introduced by Deng et al. \cite{deng2006dimensions, deng2008polynomial} as a generalisation of B-splines over hierarchical T-meshes, allowing local refinement and adaptability by means of a polynomial basis capable of parameterize the geometry. The following section briefly covers the formulation of PHT-splines.

\paragraph{T-meshes}

Let $\mathscr{T}$ be the T-mesh, $\mathscr{H}$ be the cells in $\mathscr{T}$, $\Omega \subset \mathbb{R}^2$ be the region occupied by $\mathscr{T}$. The spline space over the given T-mesh $\mathscr{T}$  is  defined as:

\begin{equation}
    \mathscr{L}(p,q,\alpha,\beta,\mathscr{T}) = \left \{ s(x,y) \in C^{\alpha,\beta}(\Omega)\left |s(x,y)  \right |_{\phi} \in\mathbb{P}_{pq} (\forall \phi \in \mathscr{H})  \right \}
\end{equation}

Where the space $\mathbb{P}_{pq}$ consists of all the bi-degree ($p,q$) polynomials and the space $C^{\alpha,\beta}$ corresponds of all the continuously bi-variate functions up to order $\alpha$ in the $x$-direction and order $\beta$ in the $y$-direction. The dimension formula of the spline space $ \mathscr{L} \left( p,q,\alpha,\beta,\mathscr{T} \right)$, when $p\geq 2\alpha +1$ and $q\geq 2\beta +1$, has already been proved in previous studies. For a $C^1$-continuous cubic spline, where every interior knots is of multiplicity two, the evaluation of the dimension formula is reduced to the following form:

\begin{equation}
    \dim\mathscr{L}(3,3,1,1,\mathscr{T}) = 4(V^b + V^+)
    \label{equation-dim-pht}
\end{equation}

Where $V^b$ and $V^+$ are boundary vertices and interior crossing vertices, respectively. \eqref{equation-dim-pht} shows that how many basis functions corresponding to the number of boundary and crossing vertices need to be constructed. It's also implied that each boundary vertex or each crossing vertex is connected by four basis functions.

\subsection{PHT-Splines Surfaces}
Let $\mathscr{T}$ be a hierarchical T-mesh, $b_{i}(\xi,\eta)$, $i=1,2,...,n$ be a set of B\'ezier splines (B-splines), $\xi$ and $\eta$ two parametric coordinates defined on the space $\left[0,1\times 0,1\right]$, and $\textbf{P}_{i}$ be the control points. Then, the polynomial spline surface over $\mathscr{T}$ at level 0 is defined by:

\begin{equation}
    \textbf{S}(\xi,\eta) = \sum_{i=1}^n b_{i}(\xi,\eta)\textbf{P}_{i} 
\end{equation}

A spline basis function can be represented locally as a linear combination of Bernstein polynomials. In particular, each B-Spline $b_{i}(\xi,\eta)$ is defined as

\begin{equation}
    b_{i} (\xi,\eta) = \sum_{j=1}^{p+1}\sum_{k=1}^{p+1}C^{i}_{jk}\hat{B}_{j,k}(\xi,\eta)
\end{equation}

\noindent where $\hat{B}_{j,k}(\xi,\eta) = B_{j}(\xi)B_{k}(\eta)$ is a tensor product of Bernstein polynomials defined on the reference interval $\left[-1,1\right]$ : 

\begin{equation}
    B_{j}(\xi) = \frac{1}{2^{p}}\binom{p}{j-1}\left(1-\xi\right)^{p-j+1}\left(1+\xi\right)^{j-1}
\end{equation}

The procedure to compute B\'ezier coefficients $C^{i}_{jk}$ based on a particular NURBS curve is detailed in \cite{borden2011isogeometric}. Then, based on a B-spline surface written over a initial regular T-mesh (level-$k$), we briefly explains how to compute the new coefficients given a refinement on a level-$k+1$: 

% Following the original definitions from \cite{deng2008polynomial}


% Let $\mathscr{T}$ be a hierarchical T-mesh, $N_{i}(\xi,\eta)$, $i=1,2,...,n$ be the basis functions, $w_{i}$ be weight functions and $\textbf{P}_{i}$ be the control points. Then, the polynomial spline surface over $\mathscr{T}$ at level 0 is defined by:

% \begin{equation}
%     \textbf{S}(\xi,\eta) = \sum_{i=1}^n R_{i}(\xi,\eta)\textbf{P}_{i} \; \; , \; \; R_{i}(\xi,\eta) = \dfrac{w_{i}N_{i}(\xi,\eta)}{\sum_{i=1}^n w_{i}N_{i}(\xi,\eta)}
% \end{equation}

% The PHT-splines at level $k$ is given as follows:

% \begin{equation}
%     \textbf{S}^k(\xi,\eta) = \sum_{i=1}^n R_{i}^k(\xi,\eta)\textbf{P}_{i}^k
% \end{equation}

% Where $R_{i}^k (\xi,\eta)$ are the same as those at level 0, but the basis functions of the PHT-splines $N_{i}^k (\xi,\eta)$ are over the hierarchical T-mesh at level-$k$ \cite{nguyen2017extended} .

% PHT-splines surfaces inherit all properties of B-splines and NURBS surfaces, and is capable to manipulate efficiently local refinement. It's in fact that PHT-splines can also be considered as a special type of Hermitian interpolation splines over T-meshes \cite{stogner2008approximation}.

\begin{enumerate}
    \item Construct a \textit{B\'ezier} representation of the basis functions. This is done using Bernstein polynomials and \textit{B\'ezier} coefficients (other authors refers them as \textit{B\'ezier} ordinates).
    \item Once a level refinement is applied, the shape functions whose support was lying on refined element must be modified. Given the B\'ezier representation of the basis function, the process consist in to truncate by zeroing out B\'ezier coefficients. This process is also explained in introductory paper to PHT-splines \cite{deng2008polynomial} and  also in the works of Garau and V\'asquez \cite{garau2018algorithms}.
    \item After the truncation of coefficients comes the insertion of new basis functions. For each new basis function, this involves the computation of the corresponding B\'ezier ordinates and the assignment of a new global basis index. We note that, the new basis functions are standard (non-truncated) B-splines, which can be computed based on local knot-vector information. In the case of a removed T-junction, the local knot-vectors need to be computed based on the neighbor connectivity of the elements which is stored in the quad-tree structure. Finally, the new basis indices corresponding to the new basis functions are determined.
\end{enumerate}

It is worth noting that, this work is based on the open-source package IGAPACK (\url{https://github.com/canitesc/IGAPack}), which already have implementations for the aforementioned routines. 


==> Sections/Sensitivity_analysis.tex <==
\subsection{Shape derivatives}
In what follows we consider a bounded open domain $\Omega \in \mathbb{R}^d (d = 2,3)$ with sufficiently smooth boundary $\partial\Omega$ and objective function $J(\Omega)$ given in either domain or boundary integral form:
\begin{equation}
    J(\Omega) = \int\limits_{\Omega}\phi(x) \, dx \label{J_domain}
\end{equation}
or
\begin{equation}
    J(\Omega) = \int\limits_{\partial\Omega}g(x) \, dS \label{J_boundary}
\end{equation}

Classical definition of shape derivative of $J(\Omega)$ (\cite{Sokolowski}, \cite{allaire:hal-02496063}) starts with introducing a small perturbation $\theta$ to domain $\Omega$:
\begin{equation}
    \Omega_{\theta} = (\text{Id} + \theta)(\Omega), \text{   where   }\theta\in\Theta_{\text{ad}}
\end{equation}
and $\Theta_{\text{ad}}$ is the space of all admissible shape variations.\\ 
Then function $J(\Omega)$ is said to be differentiable at $\Omega$ if mapping $\theta \rightarrow J(\Omega_{\theta})$ is Fr\'echet differentiable at $\theta = 0$. The shape derivative is denoted as $J'(\Omega)$ and the following equation holds:
\begin{equation}
    J(\Omega_{\theta}) = J(\Omega) + J'(\Omega)(\theta) + o(\theta)
\end{equation}

If $J(\Omega)$ is given by equation (\ref{J_domain}) then its shape derivative is
\begin{equation}
    J'(\Omega) = \int\limits_{\Omega}\text{div}(\phi(x)\, \theta) \, dx = \int\limits_{\partial\Omega}f\theta \cdot n\, dS \label{J_der_domain}
\end{equation}

If $J(\Omega)$ is given by equation (\ref{J_boundary}) then its shape derivative is
\begin{equation}
    J'(\Omega) = \int\limits_{\partial\Omega}\left(\dfrac{\partial g}{\partial n} + \kappa g\right)\theta \cdot n\, dS \label{J_der_domain_2}
\end{equation}
where $\kappa$ is the mean curvature. 

In the applications, considered in this work, objective function depends not only on the domain but also on the quantity of interest, which is required to satisfy the governing boundary value problem. Let us consider domain $\Omega$ with boundary $\partial\Omega$ and the functional
\begin{equation}
    J(\Omega) = \int\limits_{\Omega}j(u_{\Omega})dx,
\end{equation}
where $j: \mathbb{R}\rightarrow\mathbb{R}$ and $u_{\Omega}$ satisfies Neumann boundary value problem:
\begin{equation}
\begin{split}
    \Delta u + k^2 u &= f \text{   in  }\Omega\\
    \dfrac{\partial u}{\partial n} &= 0 \text{   on  } \partial\Omega\\
\end{split}\label{BVP-strong}
\end{equation}
Boundary value problem (\ref{BVP-strong}) corresponds to the weak form:
\begin{equation}
    a(u, v) = l(v),  \text{   }\forall{v}\in H_{1}(\Omega)
\end{equation}
where
\begin{equation}
    a(u, v) = \int\limits_{\Omega}(-\nabla u \nabla v + k^2 u\, v) dx
\end{equation}
\begin{equation}
    l(v) = \int\limits_{\Omega}fv dx
\end{equation}
For derivation of shape derivatives, we will use Ch\'{e}a's method, based on the following Lagrangian functional:
\begin{equation}
    \mathcal{L}: \mathcal{U_\text{ad}}\times H^1(\mathbb{R}^d) \times H^1(\mathbb{R}^d)
\end{equation}
defined as
\begin{equation}
\begin{split}
    \mathcal{L}(\Omega, u, p) &= \int\limits_{\Omega}j(u)dx +
    \int\limits_{\Omega}(\Delta u + k^2 u - f)p \, dx\\
                              &= \int\limits_{\Omega}\left(j(u) -\nabla u \cdot \nabla p + k^2 u p - f p \right) dx \\
                              &= \int\limits_{\Omega}j(u)dx + a(u, p) - l(p) \\
\end{split}
\end{equation}
From the definition of $\mathcal{L}(\Omega, u, p)$ it is evident that
\begin{equation}
    J(\Omega) = \mathcal{L}(\Omega, u_{\Omega}, p),  \text{   }\forall{p}\in H_{1}(\Omega)
\end{equation}
In what follows, we will need Green's identities:
\begin{equation}
    \int\limits_{\Omega}(p\,\Delta u - \Delta p\,u)dx = \int\limits_{\partial\Omega}\left(\dfrac{\partial u}{\partial n} p - \dfrac{\partial p}{\partial n} u \right)dS
\end{equation}
and
\begin{equation}
    \int\limits_{\Omega}\Delta u \,p \,dx = \int\limits_{\Omega}-\nabla u \nabla p \, dx + \int\limits_{\partial\Omega}\dfrac{\partial u}{\partial n} p\,dx
\end{equation}
For a given $\Omega \in \mathcal{U}_{\text{ad}}$, we are interested in stationary points $(u, p)$ of $\mathcal{L}(\Omega, u, p)$, i.e. those where
\begin{equation}
    \dfrac{\partial \mathcal{L}}{\partial u}(\Omega, u, p) = \dfrac{\partial \mathcal{L}}{\partial p}(\Omega, u, p) = 0
\end{equation}
Derivative of $\mathcal{L}(\Omega, u, p)$ with respect to $p$ is:
\begin{equation}
    \dfrac{\partial \mathcal{L}}{\partial p}(\Omega, u, p)(\hat{p}) = \int\limits_{\Omega}(\Delta u + k^2 u - f)\hat{p} \, dx = 0 \qquad\qquad\forall{\hat{p}}\in H_{1}(\Omega)
\end{equation}
which yields state equation (\ref{BVP-strong}).
In order to take derivative of $\mathcal{L}(\Omega, u, p)$ with respect to $u$ we write $\mathcal{L}(\Omega, u, p)$ as
\begin{equation}
\begin{split}
\mathcal{L}(\Omega, u, p) &= \int\limits_{\Omega}j(u)dx + \int\limits_{\Omega}(\Delta u + k^2 u - f)p \, dx \\
&=  \int\limits_{\Omega}j(u)dx + \int\limits_{\Omega}\Delta u\, p\, dx + \int\limits_{\Omega}(k^2 u - f)p \, dx \\
&= \int\limits_{\Omega}j(u)dx + \int\limits_{\Omega}\Delta p\, u\, dx + \int\limits_{\partial\Omega}\left(\dfrac{\partial u}{\partial n} p - \dfrac{\partial p}{\partial n} u \right)dS + \int\limits_{\Omega}(k^2 u - f)p \, dx \\
\end{split}\label{der_L_der_u}
\end{equation}

Then
\begin{equation}
    \dfrac{\partial \mathcal{L}}{\partial u}(\Omega, u, p)(\hat{u}) = \int\limits_{\Omega}j'(u)\hat{u}\, dx + \int\limits_{\Omega}(\Delta p + k^2 p)\, \hat{u}\, dx\qquad\qquad\forall{\hat{u}}\in H_{1}(\Omega)
\end{equation}
where the third term in (\ref{der_L_der_u}) disappears if 
\begin{equation}
    \dfrac{\partial u}{\partial n} = \dfrac{\partial p}{\partial n} = 0
\end{equation}
Hence, the adjoint equation is given by:
\begin{equation}   
\begin{split}
    \Delta p + k^2 p &= -j'(u)\\
    \dfrac{\partial p}{\partial n} &= 0
\end{split}\label{BVP-strong-adjoint}
\end{equation}
and its unique solution is denoted by $p_{\Omega}$. Next, if $u =  u_{\Omega}$ and $p = p_{\Omega}$, shape derivative of $\mathcal{L}(\Omega, u, p)$ is given by:
\begin{equation}
    J'(\Omega) = \dfrac{\partial \mathcal{L}}{\partial \Omega}(\Omega, u_{\Omega}, p_{\Omega})(\theta) = \int\limits_{\partial\Omega}\left(j(u_{\Omega}) - \nabla u_{\Omega} \cdot \nabla p_{\Omega} + k^2 u_{\Omega} p_{\Omega} - f p_{\Omega}\right)\theta \cdot n\, dS,
\end{equation}
as follows directly from eq.(\ref{J_der_domain}).


==> Sections/Shape-optimization/Shape-optimization-review.tex <==
\subsection{Overview}


==> Sections/Time-harmonic-acoustics/BVP-main.tex <==
\begin{tikzpicture}[scale = 1, classical/.style={thick, ->,>=stealth}]
\draw [black, thick] plot [smooth cycle] coordinates {(2,0) (2.25, 1) (1.5,2) (0,1) (-1,1.5) (-2,1.5) (-2.25,0.75) (-1.75,0) (-1.5, -0.75) (-1.75, -1.25) (-0.75, -1.55) (0,-1.5) (1, -1) (2,-1.25)};

\node[] at (0, 0) {$\Omega$};

\node[] at (-2.25, 1.75) {$\Gamma_N$};

\node[] at (2.0, 2.25) {$\Gamma_D$};

\node[] at (1.5, -1.5) {$\Gamma_R$};

\end{tikzpicture}

==> Sections/Time-harmonic-acoustics/Helmholtz.tex <==
In what follows we will consider domain $\Omega\in\mathbb{R}^d(d = 2,3)$ with sufficiently smooth boundary $\partial\Omega$ divided into three parts: $\Gamma_D$, $\Gamma_N$ and $\Gamma_R$ ($\partial\Omega = \Gamma_D \cup \Gamma_N \cup \Gamma_R$) with Dirichlet, Neumann and Robin boundary conditions respectively, as shown in Fig.\ref{fig:BVP-main}. 
\begin{figure}[!ht]
\centering
\input{Sections/Time-harmonic-acoustics/BVP-main.tex}
\caption{The acoustic problem.}\label{fig:BVP-main}
\end{figure}

The boundary value problem for the Helmholtz equation consists in finding the acoustic pressure $u$, which satisfies the Helmholtz equation in $\Omega$ and the boundary conditions on $\partial\Omega$:

	\begin{equation}  \label{eq:1}
		\triangle u + k^2u = f\;\;\;\;\;\;\;\;\;\;\;\;\text{in} \;\; \Omega   
	\end{equation}
	\begin{equation}   \label{eq:2}
	 u = g_1                 \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \;\; \;\; \;\; \; \; \; \text{on} \; \Gamma_D
	\end{equation}
	\begin{equation}      \label{eq:3}
	\frac{ \partial u}{ \partial n} = g_2      \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \;\; \;\; \; \; \; \text{on} \;  \Gamma_N
	\end{equation}
		\begin{equation}      \label{eq:4}
	\frac{ \partial u}{ \partial n} + \mathcal{B} u = g_3    \;\;\;\;\;\;\;\; \;\; \; \; \; \;\text{on} \;  \Gamma_R
	\end{equation}
	
% 	 \begin{equation}
%     \begin{array}{l l l l l l}
%       u & = & g_1 & \text{on}  & \Gamma_{D}  \\[8pt]
%       \dfrac{\partial u}{\partial n} & = & g_2 & \text{on}  & \Gamma_{N} \\[8pt]
%       \dfrac{\partial u}{\partial n} + \mathcal{B} u & = & g_3 & \text{on}  & \Gamma_{R} 
      
%     \end{array} 
%     \label{eqn:Boundary_conditions_DNR}
%     \end{equation}
 
	
	where $f$ is the source function, $g_1$ - prescribed pressure of the acoustic wave, $g_2$ - prescribed normal derivative (i.e. the normal velocity of the acoustic wave), and $g_3$ - prescribed Robin condition for some operator $\mathcal{B}$. If the problem is formulated in an exterior domain, additionally, Sommerfeld radiation condition needs to be satisfied at $r\rightarrow\infty$:
	
	\begin{equation}
	    \lim\limits_{r\rightarrow\infty} r^{\frac{d - 1}{2}}\left(\dfrac{\partial}{\partial r} - i k\right)u = 0
	\end{equation}
	
	Often, in acoustic problems in exterior domain, $u = u^s$ represents an acoustic field, induced by an incoming wave $u^{\text{inc}}$ and scattered by an object $D$ (one or many), as shown in Fig. \ref{fig:scattering}. In this case, boundary conditions on the scatterer's boundary are given as
	
	\begin{equation}   \label{eq:2}
	 u = u^{\text{inc}}                \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \;\; \;\; \;\; \; \; \; \text{on} \; \Gamma_D
	\end{equation}
	\begin{equation}      \label{eq:3}
	\frac{ \partial u}{ \partial n} = -\dfrac{\partial{u^{\text{inc}}}}{\partial n}     \;\;\;\;\;\;\;\;\;\;\;\;\;\;\;\; \;\; \;\; \; \; \; \text{on} \;  \Gamma_N
	\end{equation}

For numerical simulations, exterior domain is truncated by an artificial boundary $\Sigma$, where the Sommerfeld radiation condition is approximated by a so-called Absorbing Boundary Condition (ABC):	
	\begin{equation}      \label{eq:4}
	\frac{ \partial u}{ \partial n} + \mathcal{B} u = 0    \;\;\;\;\;\;\;\; \;\; \; \; \; \;\text{on} \;  \Sigma
	\end{equation}
A several types of ABCs will be discussed in Section \ref{trunc-domain-chapter}.	
\begin{figure}[!ht]
\centering
\input{Sections/Time-harmonic-acoustics/scattering_figure}
\caption{Scattering problem: given incoming wave $u^{\text{inc}}$ and the scatterer, find scattered wave $u^s$} \label{fig:scattering}
\end{figure}

\subsection{Shape optimization problem}
The first class of problems, considered in this work, is shape optimization problems. The aim of shape optimization is to improve acoustic performance of the system by modifying the boundary of the structure. Improving acoustic performance is achieved by minimizing certain quantity of interest $J(u_{\Omega})$ (e.g. level of sound in the protected zone) subjected to some design constrains. Notation $J(u_{\Omega})$ implies that $J$ is function of the solution of the Helmholtz boundary value problem $u_{\Omega}$, which in its term depends on domain $\Omega$, where the problem is solved. One of the main feature of spline-based boundary parameterization used in this work is that the boundary is described by a set of control points $\boldsymbol{x}$, which are used as design variables. Hence, the problem is written as follows:
\begin{equation}
\begin{split}
    \text{Objective function:   }& \min\limits_{\boldsymbol{x}} J(u_{\Omega}), \text{   subject to eq.(1) - (4)}\\
    \text{Such that:   }& a_i \leq x_i \leq b_i, \\
    \text{             }& f(\boldsymbol{x}) = 0, \\
    \text{             }& g(\boldsymbol{x}) \leq 0, \\
\end{split}
\end{equation}
where each design variable $x_i$ is set to take values within interval $[a_i, b_i]$,  and functions $f(\boldsymbol{x})$ and $g(\boldsymbol{x})$ represents a non-linear constraint, such as design limit on the area or volume of the structure. 

\subsection{Scatterer shape reconstruction problem}
The second class of problems, considered in this work is scatterer shape reconstruction problems. Such problems consist in finding the shape of the scatterer from a set of measurements. It can be formulated as optimization problem if the objective function is set to be the difference between the numerical simulation ($u^{s}$) and the measured data ($u^{m}$):
\begin{equation}
J(u^{s}) = \dfrac{1}{2}\int\limits_{S}|u^{s} - u^{m}|^2 dS, \label{inverse_eq}
\end{equation}
where $S$ is the surface where the measurements are taken. This type of problems is closely related to shape optimization problems in structural analysis and can be treated by the same methods. 
\begin{figure}[!ht]
\centering
\input{Sections/Time-harmonic-acoustics/scattering_figure_inverse}
\caption{Inverse scattering problem: given incoming wave $u^{\text{inc}}$ and measured wave $u^{m}$ at surface $S$, find the shape of the scatterer}\label{fig:scattering_inverse}
\end{figure}

\subsection{Sound source reconstruction problem}
The third class of problems considered in this work is source reconstruction problems. 

==> Sections/Time-harmonic-acoustics/scattering_figure.tex <==
\begin{tikzpicture}[scale = 1, classical/.style={thick, ->,>=stealth}]
\draw [black, thick] plot [smooth cycle] coordinates {(0,1) (1,2) (2,2) (1.5,1) (1.75,0.5)};
\draw [black, thick] plot [smooth cycle] coordinates {(-0.75,-0.75) (-0.5,0.25) (0.5,0) (1.,-0.75) (0.75,-1.25)};
\draw [black, thick] plot [smooth cycle] coordinates {(1.5 - 0.25,-0.75) (1.75 - 0.25,0.25) (2 - 0.25,-1+1) (2.25 - 0.25,-0.75) (2.5- 0.25,-1.25) (2.25 - 0.25,-1.5)};
\draw[classical] (-3,0) -- (-2,0)  node[midway,above] {$u^{\text{inc}}$};
\draw[thick] (-2.75,-0.1)--(-2.75,0.1) ;
\draw[thick] (-2.7,-0.1)--(-2.7,0.1) ;

\draw[classical] (3,0) -- (4,0)  node[midway,above] {$u^{\text{s}}$};
\draw[thick] (3.2,-0.1)--(3.2,0.1) ;
\draw[thick] (3.25,-0.1)--(3.25,0.1) ;

\draw[classical, rotate = 25] (3,0) -- (4,0)  node[midway,above] {$u^{\text{s}}$};
\draw[thick, rotate = 25] (3.2,-0.1)--(3.2,0.1) ;
\draw[thick, rotate = 25] (3.25,-0.1)--(3.25,0.1) ;

\draw[classical, rotate = -25] (3,0) -- (4,0)  node[midway,above] {$u^{\text{s}}$};
\draw[thick, rotate = -25] (3.2,-0.1)--(3.2,0.1) ;
\draw[thick, rotate = -25] (3.25,-0.1)--(3.25,0.1) ;

\node at (0,-0.5) {$D$};

\end{tikzpicture}

==> Sections/Time-harmonic-acoustics/scattering_figure_inverse.tex <==
\begin{tikzpicture}[scale = 1, classical/.style={thick, ->,>=stealth}]
\draw [thick, dashed, red] plot [smooth cycle] coordinates {(-1,0.5) (1,1.5) (2,0.5) (2,0) (1.5,-0.5)};

\draw[classical] (-3,0) -- (-2,0)  node[midway,above] {$u^{\text{inc}}$};
\draw[thick] (-2.75,-0.1)--(-2.75,0.1) ;
\draw[thick] (-2.7,-0.1)--(-2.7,0.1) ;

\draw[classical] (3,0) -- (4,0)  node[midway,above] {$u^{\text{s}}$};
\draw[thick] (3.2,-0.1)--(3.2,0.1) ;
\draw[thick] (3.25,-0.1)--(3.25,0.1) ;

\draw[classical, rotate = 25] (3,0) -- (4,0)  node[midway,above] {$u^{\text{s}}$};
\draw[thick, rotate = 25] (3.2,-0.1)--(3.2,0.1) ;
\draw[thick, rotate = 25] (3.25,-0.1)--(3.25,0.1) ;

\draw[classical, rotate = -25] (3,0) -- (4,0)  node[midway,above] {$u^{\text{s}}$};
\draw[thick, rotate = -25] (3.2,-0.1)--(3.2,0.1) ;
\draw[thick, rotate = -25] (3.25,-0.1)--(3.25,0.1) ;

\draw[dashed] (4.5,-2) arc (-25:25:5cm);
\node at (5, -2.) {$S$};
\node at (5.5, 0.) {$u^{m}$};
\end{tikzpicture}
